Studying Two-Photon Exchange in Deep Inelastic Scattering with the HERA Data

Two-photon exchange (TPE) is one of the leading explanations for discrepancies in measurements of the proton electromagnetic form factors. It has been proposed that TPE could impact not only elastic scattering, but also the cross sections for both inclusive deep inelastic scattering (DIS) and semi-inclusive DIS, thereby affecting the interpretation of DIS structure functions in terms of parton distributions. It is expected that higher-order QED effects such as TPE should manifest as a deviation from unity in the ratio of \epp and \emp DIS cross sections. We use the existing inclusive $e^{\pm}p$ DIS data from HERA and SLAC to constrain higher-order QED effects on inclusive DIS.

==> defs.tex <==
%===============================================================================
% defs.tex — common macros for physics papers
%===============================================================================
\ProvidesFile{defs.tex}[2025/06/21 v1.0 Common physics & formatting macros]

%% units
\newcommand{\GeV}{\ensuremath{\mathrm{GeV}}\xspace}
\newcommand{\GeVsq}{\ensuremath{\mathrm{GeV}^2}\xspace}
\newcommand{\MeV}{\ensuremath{\mathrm{MeV}}\xspace}
\newcommand{\TeV}{\ensuremath{\mathrm{TeV}}\xspace}

%% kinematic variables
\newcommand{\qsq}{\ensuremath{Q^2}\xspace}
\newcommand{\xbj}{\ensuremath{x_{\mathrm{Bj}}}\xspace}
\newcommand{\eps}{$\varepsilon$\xspace}

%% processes & reactions
\newcommand{\epem}{\ensuremath{e^+e^-}\xspace}
\newcommand{\epp}{\ensuremath{e^+p}\xspace}
\newcommand{\emp}{\ensuremath{e^-p}\xspace}
\newcommand{\eep}{\ensuremath{e^\pm p}\xspace}
\newcommand{\epphi}{\ensuremath{e + p \to e + p + \phi}\xspace}

%% structure functions & form-factors
\newcommand{\Fthree}{\ensuremath{F_3^{\gamma Z}}\xspace}
\newcommand{\GE}{\ensuremath{G_E}\xspace}
\newcommand{\GM}{\ensuremath{G_M}\xspace}

%% math shortcuts
\newcommand{\order}[1]{\ensuremath{\mathcal{O}\!\bigl(#1\bigr)}\xspace}
\newcommand{\dd}{\ensuremath{\,\mathrm{d}}\xspace}

%% styling & formatting
\newcommand{\figref}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\secref}[1]{Sec.~\ref{#1}\xspace}
\newcommand{\eqnref}[1]{Eq.~\eqref{#1}\xspace}

%===============================================================================

